Motif Cut Sparsifiers

A motif is a frequently occurring subgraph of a given directed or undirected graph $G$. Motifs capture higher order organizational structure of $G$ beyond edge relationships, and, therefore, have found wide applications such as in graph clustering, community detection, and analysis of biological and physical networks to name a few. In these applications, the cut structure of motifs plays a crucial role as vertices are partitioned into clusters by cuts whose conductance is based on the number of instances of a particular motif, as opposed to just the number of edges, crossing the cuts. In this paper, we introduce the concept of a motif cut sparsifier. We show that one can compute in polynomial time a sparse weighted subgraph $G'$ with only $\widetilde{O}(n/\epsilon^2)$ edges such that for every cut, the weighted number of copies of $M$ crossing the cut in $G'$ is within a $1+\epsilon$ factor of the number of copies of $M$ crossing the cut in $G$, for every constant size motif $M$. Our work carefully combines the viewpoints of both graph sparsification and hypergraph sparsification. We sample edges which requires us to extend and strengthen the concept of cut sparsifiers introduced in the seminal work of to the motif setting. We adapt the importance sampling framework through the viewpoint of hypergraph sparsification by deriving the edge sampling probabilities from the strong connectivity values of a hypergraph whose hyperedges represent motif instances. Finally, an iterative sparsification primitive inspired by both viewpoints is used to reduce the number of edges in $G$ to nearly linear. In addition, we present a strong lower bound ruling out a similar result for sparsification with respect to induced occurrences of motifs.

==> algorithm_changed.tex <==
%!TEX root = ./main.tex

\section{Overview of \parspar{}}

In this section we will develop the main algorithmic tool of this paper - a procedure we call \parspar{} (\cref{alg:par_spars}) that with high probability sparsifies any graph (with sufficiently many edges) by a constant factor while approximately maintaining the motif cut sizes for a set of motifs. 
Once we have this procedure available, we can iterate it $\Theta(\log n)$ times to obtain our final sparsifier. Details can be found in \cref{analysis_motif}.

 Let $\{\M_1, \ldots, \M_L\}$ be a set of motifs. We aim to obtain a graph $G'$ such that it is a $( \e, M_i)$-motif cut sparsifier of $G$ simultanuously for \emph{all} $M_i$, $i \in [L]$. For $i\in[L]$, denote $r_i = |V_{\M_i}|$ and $r^*_i = |E_{\M_i}|$ as the size of the vertex and edge set of the $i$-th motif respectively; denote $r_{max} = \max_{i \in [L]} r_i$, $r^*_{max} = \max_{i \in [L]} r^*_i$ as the largest $r_i$ and $r^*_i$ value among all $i \in [L]$, respectively. As we will see, the running time and the sparsifier size depends on $r_{max}$ and $r^*_{max}$.

In our proofs, we will use a sufficiently small constant $d>0$, as well a constant $c_1>0$ which will govern the success probability of the algorithm. The value of $d$ depends on $c_1$; this dependency is determined in \cref{lem:layer_concentration}. The value of $c_1$ is arbitrary; we can for example assume that $c_1 = 10$ (this would ultimately lead to the failure probability being at most $n^{-5}$).

%On top of that, because we are sparsifying the graph iteratively, in \parspar{} we will aim to construct an $(M_i, \e')$-motif cut sparsifier for all $i \in [L]$ for $\e' = \frac{\epsilon}{2 c_1 r^*_{max} \log n }$ instead of $\e$, to accommodate a gradual loss of precision.

Our procedure \parspar{} is very simple. 
It identifies a set of \emph{critical edges} that have to be included in the sparsifier as sampling them would result in too high variance. The remaining edges will be taken with probability $1/2$.
We start by introducing definitions used in the algorithm.


\begin{definition}[Motif Weight of an Edge]
Let $\mathcal M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Then the $\M$-motif weight of an edge $w_\M(e)$ is defined as \[w_\M(e) = \sum_{I \in \MG GM: e \in E(I)} w(I).\]
\end{definition}


\begin{definition}[Importance Weight]\label{def:edge_importance}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Then 
\begin{itemize}
    \item for $I \in \MG GM$ the importance weight in $G$ is $\ws(I) = w(I) / \kappa_I$,
    \item for an edge $e \in E$, the $\M$-importance weight in $G$ is \[\ws_\M(e) = \sum_{I \in \MG GM: e \in E(I)} \ws(I).\]
\end{itemize}
\end{definition}

We now formally define our notion of critical edges.

\begin{definition}[Critical Edge]
\label{def:critical}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
An edge $e$ is called $\M$-critical if the $\M$-importance weight of $e$ is at least $\frac{d \epsilon'^2}{r^* (\log n + r)}$.
\end{definition}

While it is possible to compute the strengths of all motif instances exactly, it can be computationally expensive. Instead, we will approximate them.

\begin{lemma}[Follows from Theorem 6.1 of \cite{chekuri2018minimum}, Strength Estimation]
\label{lem:strength_est}
There exists algorithm \textsc{StrengthEstimation} which does the following:
it receives as an input a directed weighted graph $G=(V,E, w)$ and a motif instance set $\MG GM$ for a motif $\M=(V_\M,E_\M)$ and outputs strength estimations $\kappa'_I$ for each motif instance $I \in \MG GM$ with the following properties:
\begin{enumerate}
    \item For all $I \in \MG GM$, $\kappa'_I \leq \kappa_I$,
    \item $\sum_{I \in \MG GM} \frac{w(I)}{ \kappa'_I} \leq cr(n - 1)$, for some constant $c > 0$
\end{enumerate}
where $r = |V_M|$.
The running time of the algorithm is $O(r|\MG GM| \log^2 n \log (r |\MG GM|))$.
\end{lemma}

We defer the discussion of this algorithm and proof of this lemma to \cref{sec:str_est}. 

Since we don't have access to the motif instance strengths in our algorithm, we need to define a version of importance weight that uses strength approximations.

\begin{definition}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Let $\kappa'_I$ be the estimations produced by the algorithm from \cref{lem:strength_est} for the graph $G$ for the motif $M$. 
\begin{itemize}
    \item For $I \in \MG GM$ the estimated importance weight is $\wse(I) = w(I) / \kappa'_I$,
    \item For an edge $e \in E$, the estimated $M$-importance weight is \[\wse_\M(e) = \sum_{I \in \MG GM: e \in E(I)} \wse(I).\]
\end{itemize}
\end{definition}

We can now present the \cref{alg:par_spars}.

\begin{algorithm}[H]
\caption{Partial Sparsification}
\label{alg:par_spars}
\begin{algorithmic}[1]
\Procedure{\textsc{PartialSparsification}}{$V, E, w, \epsilon', \{ \MG G{M_i} \}_{i=1}^{L} $} 
\State $E_+ \gets \emptyset$
\For{$i = 1 \to L$}
\State $ \{ \kappa'_f\}_{f \in F_{M_i}} \gets \Call{StrengthEstimation}{G, \MG G{M_i}} $
\State $E_+ \gets E_+ \cup \{ e \in E_1: \wse_{\M_i}(e) \geq \frac{d \epsilon'^2}{ r^*_i (\log n + r_i) } \}$
\label{line:find_crit}
\Comment{Find critical edges}
\EndFor
\State $E_- \gets \emptyset$
\State $w'\gets w$
\For{$e\in E \setminus E_+$}
%\State \jnote{why not "with probability $p$"?}
\If{a fair coin shows head} 
\State $w'(e)\gets 2 w(e)$
\Else
\State $w'(e)\gets 0$
\State $E_-\gets E_-\cup \{e\}$
\EndIf
\EndFor
\State $E \gets E \setminus E_-$
\State \Return $(E, w')$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> analysis_partial_changed.tex <==
%!TEX root = ./main.tex

\section{Analysis of \textsc{PartialSparsification}}
In this section, we will show that \parspar{} indeed produces an $(\e', M)$-motif cut sparsifier of the input graph $G=(V,E)$.

\subsection{Algorithm \parspar{} - Analysis of $E_+$}
%\jnote{It doesn't make sense for this to be its own section. Can we move it to a subsection of the next section?}
Fix one of the motifs among $\M_1, \ldots, \M_L$ as $M$, and denote $r = |V(M)|$, $r^* = |E(M)|$. From here on we will show a number of properties of our algorithm that would eventually allow us to show that the final graph is a $M$-motif cut sparsifier. Since it will generally not involve any other motifs, we will omit mentioning $M$ in subscripts and other places where appropriate until \cref{subsec:multi_motif}.

$E_+$ is a set produced by $\parspar$. Recall that we want to sample each critical edge with probability $1$ and each other edge with probability $p$. In fact, what happens in the algorithm is that all of the edges in $E_+$ are sampled with probability $1$ and all other edges are sampled with probability $p$. Therefore, to show the correctness of the algorithm, it is necessary to show that $E_+$ contains all of the critical edges. Moreover, since on each iteration the graph loses about $1 - p$ fraction of the edges not in $E_+$, it is necessary for us to bound the number of edges in $E_+$ in order to bound the number of edges in the output graph. We do both in this section.

\cstodo{Similarly to the algorithm, $E_1$ should be $E$ in this place.}
Denote
\[E_{M+} = \left\{ e \in E_1: \wse_{\M}(e) \geq \frac{d \epsilon'^2}{ r^* (\log n + r) } \right\}.\] 
First, we show that $E_{M+}$ (and consequently $E_+$) contains all $M$-critical edges:


\begin{lemma}
\label{lem:crit_correct}
The set $E_+$ in line \ref{line:find_crit} of \cref{alg:par_spars} contains all $M$-critical edges.
\end{lemma}
\begin{proof}
By \cref{lem:strength_est},
\[
    \forall I \in \MG GM: \kappa'_I \leq \kappa_I.
\]
By definition of $M$-critical edge and importance weight,
\[
    \sum_{I \in \MG GM: e \in E(I)} \frac{w(I)}{\kappa_I} \geq \frac{d \epsilon'^2}{r^* \log n}.
\]
On the other hand,
\[
    \sum_{I \in \MG GM: e \in E(I)} \frac{w_\M(I)}{\kappa_I} \leq \sum_{I \in \MG GM: e \in E(I)} \frac{w_\M(I)}{\kappa'_I} = \wse_\M(e).
\]
Therefore, the condition in line \ref{line:find_crit} of \cref{alg:par_spars} holds for $e$, which means that $E_+$ contains all $M$-critical edges.
\end{proof}



Furthermore, we have that $E_+ = \bigcup_{i=1}^{L} E_{M_i+}$, hence by bounding $E_{M+}$ we can bound $E_+$.

\begin{lemma}
\label{lem:crit_counting}
The size of $E_{M+}$ is at most 
$\frac{c r (r^*)^2 (n - 1) (\log n + r)}{d \epsilon'^2}$.
\end{lemma}
\begin{proof}
By \cref{lem:strength_est}, the following holds:
\[
    \sum_{I \in \MG GM} \wse(I) \leq c r (n - 1).
\]
We can bound the sum of estimations of importance weight of all edges:
\[
    \sum_{e \in E} \wse_\M(e) = \sum_{e \in E} \sum _{\substack{I \in \MG GM:\\ e \in E(I)}} \wse(I) \leq
    r^* \sum_{I \in \MG GM} \wse(I) \leq c r r^* (n - 1).
\]
On the other hand, since edges in $E_{+M}$ must satisfy inequality in line \ref{line:find_crit} of \cref{alg:par_spars}, we have
\[
    |E_{M+}| \cdot \frac{d \e'^2}{r^* (\log n + r)} \leq \sum_{e \in E_{M+}} \wse_\M(e) \leq \sum_{e \in E} \wse_\M(e).
\]
Combining both inequalities yields:
\[
    |E_{M+}| \leq \frac{c r (r^*)^2 (n - 1) (\log n + r)}{d \epsilon'^2},
\]
as desired.
\end{proof}

\begin{corollary}
\label{cor:total_crit_counting}
$E_+$ satisfies
\[|E_+| \le \frac{c L r_{max} {(r^*_{max})^2} (n - 1) (\log n + r_{max})}{d \epsilon'^2}. \]
\end{corollary}
\begin{proof}
The proof follows from \cref{lem:crit_counting} by summing across all motifs.
\end{proof}







%Throughout this section we will denote by $G$ the state of the graph at the beginning of the iteration rather than beginning of an algorithm for simplicity.

\subsection{Correctness of \textsc{PartialSparsification}}

As in \cite{benczur_randomized_2015}, to show the correctness of our algorithm, we want to split our graph $G$ into a ``sum'' of several weighted graphs. The decomposition may be viewed as the motif-version of the decomposition of Benczur and Karger \cite{benczur_randomized_2015} and follows rather closely their ideas. 

Let $k_1, \ldots, k_h$ be all of the different strong $M$-connectivity values in $G$ in increasing order, i.e. for each $k_i$ there exists a $k_i$-strongly connected component that is not $k$-strongly connected for any $k>k_i$. Let $k_0 = 0$. 
In order to decompose our graph into a sum of weighted graphs we observe that we can write
\begin{eqnarray*}
\Val_{M, G}(S, V \setminus S) &=& \sum_{\substack{I \in \MG GM: \\ I \text{ crosses }(S, V \setminus S)}} w(I)\\
& = &
\sum_{\substack{I \in \MG GM: \\ I \text{ crosses } (S, V \setminus S)}} \frac{w(I)}{\kappa_I} \cdot \kappa_I \\
& = & \sum_{\substack{I \in \MG GM: \\ I \text{ crosses } (S, V \setminus S)}}
\frac{w(I)}{\kappa_I} \cdot \left(\sum_{i: k_i \le \kappa_I} k_i - k_{i-1}\right) \\
&=& \sum_{i=1}^h (k_i - k_{i-1}) \cdot 
\sum_{\substack{I \in \MG GM: \\
\kappa_I \ge k_i}} \frac{w(I)}{\kappa_I}
\cdot {\mathbbm 1}(I \text{ crosses } (S, V \setminus S))
\end{eqnarray*}
where the third equality follows from $\kappa_I = \sum_{i:\kappa_I \ge k_i} k_i-k_{i-1}$  
and where
${\mathbbm 1}(I \text{ crosses } (S, V \setminus S))$ denotes the indicator function that motif instance $I$ crosses the cut $(S,V\setminus S)$.
The above formula guides us towards our decomposition. The sum 
$$
\sum_{\substack{I \in \MG GM: \\
\kappa_I \ge k_i}} \frac{w(I)}{\kappa_I}\cdot {\mathbbm 1}(I \text{ crosses } (S, V \setminus S))
$$
ranges over all motif instances that are contained in components of $M$-connectivity at least $k_i$. We will now view the graph as a sum of graphs $F_i$ where each $F_i$ is the union of all $k_i$-strongly $M$-connected components of $G$. The motif instances in the graph $F_i$ will be weighted by a factor of $k_i-k_{i-1}$.
In addition, each motif $I$ is reweighted by $1/\kappa_I$ in all graphs $F_i$. This motivates the following definition.

%This motivates the following definition.
%The main idea is to decompose each motif instance into several instances and distribute them across all of the strongly $M$-connected component with different weights. In particular, for an instance $I$ suppose that it is contained inside components $C_1, \ldots, C_h$ of strong $M$-connectivities $k_1, \ldots, k_h$ in increasing order. Then component $C_j$ will have $I$ with weight $\frac{k_j - k_{j - 1}}{\kappa_I}$. It is easy to see that those weights sum up back to $1$, and that they are consistent across all motifs, i.e. the graph $G$ would be just the sum of all of it's connectivity components.




%Since we are working with motifs, unlike the algorithm of Benczur and Karger, we need to split each motif instance into several motif instances, where weights of each instance $I$ is modified by multiplying it by $1/\kappa_I$. But since the weights of edges are unaffected, we will instead just split the motif size of a cut into a sum of several re-weighted motif cut sizes.

\begin{definition}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w')$ be a directed weighted graph. For a subgraph $H=(V_H,E_H,w)$ of $G$ (where the weights in $H$ may differ from $G$) and a cut $(S,V_H \setminus S)$
, we define the following value:
\[
    \IVal_{M, H}(S, V_H \setminus S) = \sum_{\substack{I \in \MG HM:\\
    I \text{ crosses } (S, V_H \setminus S)}} \frac{w(I)}{\kappa_I(G)},
\]
where $\kappa_I(G)$ is the motif strength of $I$ with respect to $G$.
\end{definition}
In the following we will always use the above definition in a way that $G$ is the input graph of \parspar{}. We will also frequently use $G$ as a subscript when the subgraph $H$ in the above definition equals $G$.
Using the above notation we can now write
\begin{eqnarray}
\Val_{M, G}(S, V \setminus S) 
& =& \sum_{i=1}^h (k_i-k_{i-1}) \cdot 
  \IVal_{M, F_i}(S, V \setminus S)\\
  &=& \sum_{i=1}^h (k_i-k_{i-1}) \cdot
  \sum_{\substack{\text{ $k_i$-strongly connected}\\ \text{component } C}}  \IVal_{M, C}(S, V \setminus S)\label{eqn}
\end{eqnarray}
where the last equality splits $F_i$ into its strongly $M$-connected components.

%The plan of this section is as follows: we first show that for all strongly $M$-connected components $C$, $\IVal_{M, C}$ of each cut in them is $(1 \pm \e)$-preserved. Then, we show that a motif size of an arbitrary cut in the whole graph can be represented as a weighted sum of $\IVal_{M, C}$ of the same cut in several connectivity components $C$. Finally, combining those two results, we show that \parspar{} produces $(M, \e')$-motif cut sparsifier.

%We will start with the existence of cut decomposition. The idea is to a cut each motif instance into several instances and distribute them across all of the strongly $M$-connected component containing with different weights. In particular, for an instance $I$ suppose that it is contained inside components $C_1, \ldots, C_h$ of strong $M$-connectivities $k_1, \ldots, k_h$ in increasing order. Then component $C_j$ will have $I$ with weight $\frac{k_j - k_{j - 1}}{\kappa_I}$. It is easy to see that those weights sum up back to $1$, and that they are consistent across all motifs, i.e. the graph $G$ would be just the sum of all of it's connectivity components.

%\begin{lemma}
%\label{lem:component_sum}
%Let $C_1, \ldots, C_t$ be all of the strongly $M$-connected components of $G$, whose strengths are equal to the strength of at least one motif in $G$, in order of increasing strong $M$-connectivity. Then $t \leq 2n$ and there exists $\alpha_1, \ldots, \alpha_t \in \R$ such that for any cut $(S, V \setminus S)$,
%\[
%\Val_{M, G}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C_i}(S, V \setminus S).
%\]
%\end{lemma}
%\begin{proof}

%Note that if two strongly  $M$-connected components intersect, one of them is contained inside the other, and the smaller one has higher connectivity. Therefore, the set of all strongly $M$-connected components is a laminar family, therefore its size $t$ is at most $2n$.

%Let $k_1, \ldots, k_h$ be all of the different strong $M$-connectivity values in $G$ in increasing order, and $k_0 = 0$. For $i \in [t]$, consider the component $C_i$. Suppose that it's connectivity is $k_{h_i}$. Let $C_j$ be the minimal by inclusion component containing $C_i$, and let $k_{h_j}$ be it's strong $M$-connectivity. If it exists, we set $\alpha_i = k_{h_i} - k_{h_{j}}$, otherwise $\alpha_i = k_{h_i}$.

%Let $I \in \MG GM$ be an arbitrary motif instance. Notice that all of the strongly $M$-connected components containing $I$ must be nested. Let $k_{h_1}, \ldots, k_{h_j}$ be the strong $M$-connectivities of those components in increasing order, and let $k_{h_0} = 0$. Then $k_{h_j} = \kappa_I$. Therefore, by the assignment of $\alpha_i$, the following holds:
%\[
 %   \sum_{i: I \in \MG{C_i}{M}} \frac{\alpha_i}{\kappa_I} = \sum_{i = 1}^{j} \frac{k_{h_i} - k_{h_{i - 1}}}{\kappa_I} = 1.
%\]
%Now, consider an arbitrary cut $(S, V \setminus S)$. We have
%\begin{align*}
%    \sum_{i = 1}^{t} \alpha_i \IVal_{C_i}(S, V \setminus S)&= \sum_{i = 1}^{t} \sum_{I \in \MG {C_i}{M}: I \text{ crosses } (S, V \setminus S)}  \frac{\alpha_i \cdot  w_\M(I)}{ \kappa_I} \\
%    &= \sum_{I \in \MG {G}{M}: I \text{ crosses } (S, V \setminus S)}  w_\M(I) \sum_{i: I \in \MG{C_i}{M}} \frac{\alpha_i}{ \kappa_I}\\
%    &=\sum_{I \in \MG {G}{M}: I \text{ crosses } (S, V \setminus S)} w_\M(I) \\
%    &= \Val_{M, G}(S, V \setminus S). \qedhere
%\end{align*}
%\end{proof}

Now, our goal is to show the concentration result for a single strongly $M$-connected component.
There are two well-known results for hypergraph cuts that can be adapted for the case of motifs that we need to use to show concentration for all cuts. 
We include their proofs for completeness.

\begin{lemma}[Reformulation of Theorem 6.8 of \cite{chekuri2018minimum}]
\label{lem:weighted_cut_size}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
 If minimum of $
 \IVal_{M, G}$ of all non-trivial cuts is greater than $0$, it is equal to $1$.
\end{lemma}
\begin{proof}
\cstodo{I don't think we defined strong $M$-connectivity of a graph. Do you mean $M$-connectivity?}
Let $(S, V \setminus S)$ be the cut with minimum motif size and let $k$ be the strong $M$-connectivity of $G$. 
Then all of the motif instances crossing the cut have connectivity exactly $k$. On the other hand, the size of the cut is $k$, which gives us
\[
\IVal_{M, G}(S, V \setminus S) = 
\sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S) } \frac{w(I)}{\kappa_I} = \frac{\Val_{M, G}(S, V \setminus S)}{k} = 1. 
\]
Consider any other cut $(S, V \setminus S)$ of motif size $k'$. Then the strength of all motif instances crossing this cut is at most $k'$, which means that:
\[
\IVal_{M, G}(S, V \setminus S) = \sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S) } \frac{w(I)}{\kappa_I} \geq \frac{\Val_{M, G}(S, V \setminus S)}{k'} = 1.
\]
Therefore, the cut with the minimum motif size is the cut with the minimum value of $\IVal_{M, G}$, and the latter is equal to $1$. 
\end{proof}

\cstodo{Formulation of the lemma: Does it hold for every alpha >=1?}
\begin{lemma}[Motif Cut Counting, Reformulation of Theorem 3.2 of \cite{kogan2015sketching}]
\label{cor:cut_counting}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph. Let $c$ be the minimum value of $\IVal_{M, G}$ across all cuts in $G$. There are at most $O(2^{
(\alpha + 1) r} n^{2(\alpha + 1)})$ cuts with value $\IVal_{M, G}$ at most $\alpha c$ for a real $\alpha \geq 1$.
\end{lemma}
The proof of the above lemma is given in \cref{sec:str_est}.

In the works on graph and hypergraph sparsification 
the value of a cut is defined by the edges or hyperedges. These are also the objects that are sampled and it suffices to use a Chernoff bound to analyze the concentration of a fixed cut. In our case, we sample edges but we are interested in the number of motif instances that cross the cut. We can write the cut value as a sum of random variables corresponding to the motifs that cross the cut, but these random variables are not independent and so we cannot use Chernoff bounds. To deal with dependencies we will instead use Azuma's inequality.

\begin{lemma}[Azuma's Inequality, \cite{azuma1967weighted}]
\label{lem:azuma}
Let $Z_0, Z_1, \ldots, Z_n$ be a martingale satisfying $|Z_i - Z_{i-1}| \le c_i$ for each $i \in [n]$. For any $\lambda > 0$,
\[ \p(|Z_n - Z_0| \ge \lambda) \le 2 \exp\left( \frac{-\lambda^2}{2(c_1^2 + \cdots + c_n^2)} \right). \]
\end{lemma}
We will use this lemma with a special `edge-exposure' martingale, which will be defined in the proof of \cref{lem:layer_concentration}.

%The following lemmas use the values $\IVal_{M, G}$ in graph before and after sparsification by \parspar{}. To compute them, we only use the values of motif instance strength in the graph before the sparsification.

\begin{lemma}
\label{lem:layer_concentration}
Let $C$ be a strongly $M$-connected component before the application of \textsc{PartialSparsification} and $C'$ be that subgraph after the application. The following holds with probability at least $1 - n^{-c_1 }$:

Let $V_C = V(C)$. For all cuts $(S, V_C \setminus S)$ of $C$,
$$
    (1 - \epsilon') \IVal_{M, C}(S, V_C \setminus S) \leq \IVal_{M, C'}(S, V_C \setminus S) \leq (1 + \epsilon') \IVal_{M, C}(S, V_C \setminus S).
$$
\end{lemma}
\begin{proof}
By applying \cref{lem:weighted_cut_size} to $C$, we get that the minimum of values $\IVal_{M, C}$ across all cuts in $C$ is $1$.

Note that all of the critical edges in $C$ are critical in $G$, since their $M$-importance weight in $C$ is not larger than in $G$.
Since, by \cref{lem:crit_correct}, $E_+$ contains all critical edges in $G$, it also contains all of the critical edges in $C$, and, therefore, no critical edges are being sampled afterwards.
Fix a cut $(S,V_C\setminus S)$ with $\IVal_{M, C}(S,V_C\setminus S)=\alpha \geq 1$ in $C$. Let $E_2$, $t:=|E_2|$, be the set of all edges that are being sampled in \textsc{PartialSparsification} with probability $1/2$ and that are part of at least one motif cut by $(S, V_C \setminus S)$. Then $E_2$ does not contain any critical edges. Let $I_0$ be the subgraph of $C$ containing all vertices and edges that are a part of some motif  that is being cut by $(S, V_C \setminus S)$.

Consider the following random process: enumerate the edges in $E_2$ in the order they are being examined by \textsc{PartialSparsification}. Suppose edge $e$ with number $i$ is being sampled. If $e$ is not sampled, then we define $I_i$ to be equal to $I_{i-1}$ without $e$, otherwise $I_i$ is equal to $I_{i-1}$ with $e$ with it's weight multiplied by $2$. Now consider a random process $X_i$, $i \in \{0, \ldots, t\}$, where $X_i$ is equal to $\IVal_{M, I_i}(S, V_C \setminus S)$. 

It is easy to see that $X_t = \IVal_{M, C'}(S, V_C \setminus S)$ and that $X_i$ is a martingale. Let 
\[
\M^S(e) = \sum_{\substack{I\in\MG{C}{M}:\\ e \in E(I),\\ I \text{ crosses } (S, V_C \setminus S) }} \frac{w_\M(I)}{\kappa_I}.
\]
Then $|X_i - X_{i - 1}| \leq 2 \cdot \M^S(e)$, where $e$ is the edge being sampled on step $i$, since the weight of all motifs can change by at most a factor of $2$ during the random process. Therefore, to apply \cref{lem:azuma}, we need to bound $\sum_{e \in E_2} \M^S(e)^2$.

Since there are no critical edges in $E_2$, for all edges $e$ that we sample, we must have 
\[\M^S(e) \leq \frac{d \epsilon'^2}{r^* (\log n + r)}.\] 
On the other hand,
\[
    \sum_{e \in E_2} \M^S(e) \leq r^* \sum_{I\in\MG{C}{M}: I \text{ crosses } (S, V_C \setminus S) } \frac{w_\M(I)}{\kappa_I} = r^* \alpha,
\]
since every motif contains at most $r^*$ edges. Therefore, using this inequality:
\[  
\sum_{e \in E_2} \M^S(e)^2 \le \frac{d \epsilon'^2 }{r^* (\log n + r)} \sum_{e \in E_2} \M^S(e) \le \frac{\alpha d \epsilon'^2 }{\log n + r}.
\]
Hence, because $\IVal_{M,C}(S, V_C \setminus S) = \alpha$ and by \cref{lem:azuma},
\begin{align*}
    &\p(|\IVal_{M,C}(S, V_C \setminus S) - \IVal_{M,C'}(S, V_C \setminus S)| \geq \epsilon' \IVal_{M,C}(S, V_C \setminus S)) \leq \p(|X_t - X_0| \ge \epsilon' \alpha)  \\
    &\le 2 \exp\left( \frac{-(\epsilon' \alpha )^2}{2\sum_{e \in E_2}\M^S(e) / (1/2)} \right) \le 2 \exp\left( \frac{-(\epsilon' \alpha)^2}{4 \cdot \frac{\alpha d \epsilon'^2 }{\log n + r}} \right) = 2 \exp\left( \frac{-\alpha (\log n + r)}{4 d} \right).
\end{align*}

We now apply a union bound on all cuts $(S, V_C \setminus S)$ in conjunction with \cref{cor:cut_counting}. We need to bound $\sum_{\alpha \geq 1} P(\alpha)g(\alpha)$, where $P(\alpha)$ is the probability that the inequalities in the statement of the lemma doesn't hold for the cut with $\IVal_{M, C}$ equal to $\alpha$, $g(\alpha)$ is the number of those cuts, and the sum is taken across all values of $\alpha$ that are present in the graph.

Let $F(\alpha) = \sum_{\alpha \geq \alpha' \geq 1} g(\alpha')$ be the total number of cuts with $\IVal_{M, C} \leq \alpha$. By \cref{cor:cut_counting}, $F(\alpha) = A 2^{(\alpha + 1)r} n^{2(\alpha + 1)}$ for some constant $A$. We then adversarially extend $F(\alpha)$ in a to the whole $\R_+$ such that $F(\alpha)$ is differentiable while preserving the above inequality.

We have that
\[
\sum_{\alpha \geq 1} P(\alpha)g(\alpha) \leq \int_{1}^\infty P(\alpha) \frac{dF(\alpha)}{d\alpha} d \alpha.
\]
Therefore, by applying partial integration,
\begin{align*}
&\int_{1}^\infty P(\alpha) \frac{dF(\alpha)}{d\alpha} d \alpha = \Big[ P(\alpha) F(\alpha)  \Big]_{1}^{\infty} - \int_{1}^\infty F(\alpha) \frac{dP(\alpha)}{d\alpha} d \alpha\\
&\leq 2 A 2^{2r} n^4 \exp \left(-\frac{\log n + r}{4d}\right) + 
\int_{1}^\infty A n^{2(x + 1)} 2^{r(x + 1)} \frac{\log n + r}{4d} 2\exp \left(-\frac{x (\log n + r)}{4d} \right) dx \\
&\leq n^{-c_1 }
\end{align*}
by setting $d$ to be sufficiently small. Thus, the inequalities in the lemma statement hold with probability at least $1 - n^{-c_1 }$ for all cuts, as desired.
\end{proof}

We will now use the fact that for a given cut, we can take the weighted sum of the $\IVal_{M, C}$ of cuts of each of the connectivity components $C$ such that this sum is equal to the motif cut size in the whole graph. We can then apply \cref{lem:layer_concentration} to each term to obtain the cut preservation property for the whole graph.

\begin{lemma}
\label{lem:cut_component_preservation}
Let $G'$ be $G$ after the application of \textsc{PartialSparsification}. $G'$ is $(M, \e')$-motif cut sparsifier of $G$ with probability $1 - n^{-c_1 + 3}$.

\end{lemma}
\begin{proof}
By definition of motif cut sparsifier, it is enough to show that the following holds for all cuts $(S, V \setminus S)$ of $G$:
\[
    (1 - \epsilon')\textup{Val}_{M, G}(S, V \setminus S) \leq \textup{Val}_{M, G'}(S, V \setminus S) \leq (1 + \epsilon') \textup{Val}_{M, G}(S, V \setminus S).
\]
By equation (\ref{eqn}),  we have 
%$t \leq 2 n$ and there exist $\alpha_i \in \R$, $i \in [t]$, such that for any cut $(S, V \setminus S)$,
\begin{eqnarray*}
\Val_{M, G}(S, V \setminus S) 
  &=& \sum_i (k_i-k_{i-1}) \cdot
  \sum_{\substack{\text{ $k_i$-strongly connected}\\ \text{component } C}}  \IVal_{M, C}(S, V \setminus S).
%\textup{Val}_{M, G}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C_i}(S, V \setminus S).
\end{eqnarray*}
Now let $C'$ be $C$ after the application of \textsc{PartialSparsification}.
Then, similarly, the following holds:
\begin{eqnarray*}
\Val_{M, G'}(S, V \setminus S) 
 &=& \sum_i (k_i-k_{i-1}) \cdot 
\sum_{\substack{\text{ $k_i$-strongly connected}\\ \text{component } C \text{ in } G}} \IVal_{M,C'}(S,V\setminus S).
%\sum_{\substack{I \in \MG {C'}M: \\ I \text{ crosses } (S, V \setminus S)}} \frac{w(I)}{\kappa_I(G)}
%\textup{Val}_{M, G}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C_i}(S, V \setminus S).
\end{eqnarray*}
%\[
%\Val_{M, G'}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C'_i}(S, V \setminus S).
%\]
Note that if two strongly  $M$-connected components intersect, one of them is contained inside the other, and the smaller one has higher connectivity. Therefore, the set of all strongly $M$-connected components is a laminar family, which means that its size is at most $2n$.
By applying \cref{lem:layer_concentration} to all $k_i$-strongly $M$-connected components $C$ for all $i$ and a union bound over the at most $2n$ different strongly $M$-connected components,  the following holds for all strongly $M$-connected components:
\[
    (1 - \epsilon')\IVal_{M, C'}(S, S \setminus V) \leq \IVal_{M, C}(S, S \setminus V) \leq (1 + \epsilon') \IVal_{M, C'}(S, S \setminus V)
\]
with probability at least $1 -  2 n^{-c_1 + 1} \geq 1 -  n^{-c_1 + 3}$.
Combining all of the equalities and inequalities, we get the claim.
\end{proof}

\subsection{Hypergraphs}
We introduce hypergraphs here since we will use some results concerning them. A hypergraph is the pair of two sets $(V, F)$, where $V$ is the set of vertices and $F$ is the set of hyperedges $f$, which are subsets of $V$. A weighted hypergraph $H=(V, F, w)$ is a hypergraph with a weight function $w: F \to \R_+$.
A hypergraph $H$ is $r$-uniform if every $f \in F$ satisfies $|f| = r$.
We denote the size of the cut $(S, V \setminus S)$ in hypergraph $H$ as $\textup{Val}_H(S, V \setminus S)$.

\begin{definition}[Induced Subhypergraph]
A hypergraph $H'=(V', F', w')$ is an induced subhypergraph of a hypergraph $H=(V, F, w)$, if $V' \subseteq V$, $F' = \{ f \in F: f \subseteq V' \}$ and $w$ and $w'$ are equal on $F'$.
\end{definition}

We will abuse the cut notation for the hypergraphs: if $H'=(V', F', w)$ is an induced subhypergraph of $H=(V, F, w)$, then $\textup{Val}_{H'}(S, V \setminus S) := \textup{Val}_{H'}(S \cap V', V' \setminus S)$.

\cstodo{Why do we call it strong connectivity at this place? We call the equivalent for motifs just connectivity.}

\begin{definition}[Strong Connectivity]
A weighted hypergraph $H=(V,F,w)$ is $k$-strongly connected if 
every cut $(S,V\setminus S$), $S\neq \emptyset$, $S\subsetneq V$, in $H$ has size at least $k$.
\end{definition}
 
\begin{definition}[Strongly $k$-connected Component]
\label{def:hyper-kconnectedcomp}
For a weighted hypergraph $H=(V, F, w)$ with non-negative hyperedge weights and a value $k\in \R_+$, an induced subhypergraph $C=(V_C,F_C, w)$ of $H$ is called a strongly $k$-connected component of $H$,
if 
\begin{enumerate}[label=(\alph*)]
    \item $C$ is strongly $k$-connected and,
    \item there is no induced subhypergraph $C'=(V_{C'},F_{C'}, w)$ of $G$ that is strongly $k$-connected and has $V_C \subsetneq V_{C'}$.
\end{enumerate}
\end{definition}

\begin{definition}[Hyperedge Strength]
Let $H=(V, F, w)$ be a weighted hypergraph with non-negative hyperedge weights. A hyperedge $f \in F$ has strength $\kappa_f$ if $\kappa_f$ is the
maximum value of $k$ such that there exists a strongly $k$-connected component of $H$ that contains $f$.
\end{definition}

\subsection{Strength Estimation and Motif Cut Counting}
\label{sec:str_est}
To reiterate, construction of motif cut sparsifier is not possible by only using the techniques for constructing hypergraph sparsifier. But, the problems are sufficiently close to share some similarities, which allows us to use some results for hypergraph cut sparsification in our proof.

In this section we will present omitted proofs of \cref{lem:strength_est} and \cref{cor:cut_counting} by reducing them to similar existing results for hypergraphs.

Because motif instances are essentially just subsets of vertices, it is useful to consider them as hyperedges of some hypergraph, which we will call a motif hypergraph. Note that some motif instances share the same set of vertices. In this case, the weight of the resulting hyperedge is equal to the sum of their weights.

\begin{definition}[Motif Hypergraph]
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Then the $\M$-motif hypergraph of $G$ is an undirected weighted hypergraph $H_\M=(V, F_\M, w_\M)$, where
\begin{itemize}
    \item $F_M = \{ V(I): I \in \MG GM \}$,
    \item for $f \in F_M$, $w_M(f) = \sum_{I \in \MG G M: f = V(I)} w(I)$.
\end{itemize}
\end{definition}

Note that the motif hypergraph represents the motif connectivity structure of a graph: for a cut $(S, V \setminus S)$ in $G$, its motif size is equal to it's size in $H$, and for a $I \in \MG GM$, $\kappa_I = \kappa_{V(I)}$ where $V(I)$ is a hyperedge of motif hypergraph. The introduction of hypergraph allows us to use several results from hypergraph cut sparsification, as well as giving a new perspective on the problem.

% \begin{lemma}
% \label{lem:spars_def_alt}
% Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ and $G'=(V, E', w')$ be directed weighted graphs.
% Let $H$ and $H'$ be the $M$-motif hypergraphs of $G$, $G'$.
% $G'$ is $(M, \e)$-motif cut sparsifier iff for any cut $(S, V \setminus S)$ of $H$ the following holds:
% \[
%     (1 - \epsilon) \textup{Val}_{H}(S, V \setminus S) \leq \textup{Val}_{H'}(S, V \setminus S) \leq (1 + \epsilon) \textup{Val}_{H}(S, V \setminus S).
% \]
% \end{lemma}
% \begin{proof}
% The lemma follows from the fact that the motif size of the cut $(S, V \setminus S)$ in $G$ is equal to the size of this cut in $H$, and same for the $G'$ and $H'$.
% \end{proof}

We now prove \cref{lem:strength_est} by using the following result.

\begin{lemma}[Theorem 6.1 of \cite{chekuri2018minimum}, Strength Estimation]
\label{lem:strength_est_hyper}
There exists algorithm \textsc{StrengthEstimation} which does the following:
it receives as an input a rank $r$ weighted hypergraph $H=(V, F, w)$ on $n$ vertices and outputs strength estimations $\kappa'_f$ for each hyperedge $f$ with the following properties:
\begin{enumerate}
    \item For all $f \in F$, $\kappa'_f \leq \kappa_f$,
    \item $\sum_{f \in F} \frac{w(s)}{ \kappa'_f} \leq cr(n - 1)$, for some constant $c > 0$.
\end{enumerate}
The running time of the algorithm is $O(r|F| \log^2 n \log (r |F|))$.
\end{lemma}



Note that although the algorithm presented in \cite{chekuri2018minimum} can only work with natural weights, we can easily reduce the general case to it by dividing all of the weights by the minimum one and then rounding them down to the nearest integer: tt only worsens the second property by a factor of $2$.

\begin{proof}[Proof of \cref{lem:strength_est}]
We construct motif hypergraph $H_M$ and run the algorithm from \cref{lem:strength_est_hyper} on it, then set $\kappa'_I := \kappa'_{V(I)}$ for $I \in \MG GM$. Since the construction of $H_M$ takes only $O(|\MG GM|)$ time, the total runtime is the same as in \cref{lem:strength_est_hyper}, and both properties straightforwardly follow from properties of $H_M$.
\end{proof}

Finally, we give the proof of \cref{cor:cut_counting}.

\begin{lemma}[Cut Counting in Hypergraphs, Theorem 3.2 of \cite{kogan2015sketching}]
\label{lem:cut_counting_hyper}
In an $r$-uniform weighted hypergraph $H=(V, M, w)$ with size of minimum cut $c$, there are at most $O(2^{
\alpha r} n^{2\alpha})$ cuts of size no more than $\alpha c$ for a half-integer $\alpha \geq 1$ where $\alpha$ is a half-integer if $2 \alpha$ is an integer.
\end{lemma}

\begin{proof}[Proof of \cref{cor:cut_counting}]
Consider a modification of a motif hypergraph, where each hyperedge's weight is divided by its strength. Denote it by $H'$.
It is easy to see that the size of an arbitrary cut $(S, V \setminus S)$ in $H'$ is equal to the $\IVal_{M, G}(S, V \setminus S)$. 
Indeed, 
\begin{align*}
     \Val_{H'}(S, V \setminus S) &= \sum_{f \in F: f \text{ crosses } (S, V \setminus S)} \frac{w_M(f)}{\kappa_f} \\
    &=\sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S)} \frac{w(I)}{\kappa_I} \\
    &= \IVal_{M, G}(S, V \setminus S).
\end{align*}
Therefore, it is enough to show that if $c$ is the size of the smallest cut in $H'$, the number of cuts of size $\alpha c$ is at most $O(2^{(\alpha + 1)r}n^{2(\alpha + 1)})$, which we achieve as follows: find the smallest half integer $\beta \geq \alpha$ and apply \cref{lem:cut_counting_hyper} to it and $H'$. The result then follows from the fact that $\beta < 1 + \alpha$.
\end{proof}


==> old_analysis.tex <==


\section{OLD ANALYSIS}



\section{Analysis of \textsc{PartialSparsification}}
In this section, we will show that \parspar{} indeed produces an $(\e', M)$-motif cut sparsifier of the graph from the previous iteration.
\todo{}
Throughout this section we will denote by $G$ the state of the graph at the beginning of the iteration rather than beginning of an algorithm for simplicity.

\subsection{Correctness of \textsc{PartialSparsification}}

As in \cite{benczur_randomized_2015}, to show the correctness of our algorithm, we want to split our graph $G$ into sum of several weighted graphs. Since we are working with motifs, unlike the algorithm of Benczur and Karger, we need to split each motif instance into several motif instances, where weights of each instance $I$ is modified by multiplying it by $1/\kappa_I$. But since the weights of edges are unaffected, we will instead just split the motif size of a cut into a sum of several re-weighted motif cut sizes.

\begin{definition}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph. For a cut $(S, V \setminus S)$, we define the following value:
\[
    \IVal_{M, G}(S, V \setminus S) = \sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S)} \frac{w(I)}{\kappa_I}.
\]
\end{definition}

The plan of this section is as follows: we first show that for all strongly $M$-connected components $C$, $\IVal_{M, C}$ of each cut in them is $(1 \pm \e)$-preserved. Then, we show that a motif size of an arbitrary cut in the whole graph can be represented as a weighted sum of $\IVal_{M, C}$ of the same cut in several connectivity components $C$. Finally, combining those two results, we show that \parspar{} produces $(M, \e')$-motif cut sparsifier.

We will start with the existence of cut decomposition. The idea is to a cut each motif instance into several instances and distribute them across all of the strongly $M$-connected component containing with different weights. In particular, for an instance $I$ suppose that it is contained inside components $C_1, \ldots, C_h$ of strong $M$-connectivities $k_1, \ldots, k_h$ in increasing order. Then component $C_j$ will have $I$ with weight $\frac{k_j - k_{j - 1}}{\kappa_I}$. It is easy to see that those weights sum up back to $1$, and that they are consistent across all motifs, i.e. the graph $G$ would be just the sum of all of it's connectivity components.

\begin{lemma}
\label{lem:component_sum}
Let $C_1, \ldots, C_t$ be all of the strongly $M$-connected components of $G$, whose strengths are equal to the strength of at least one motif in $G$, in order of increasing strong $M$-connectivity. Then $t \leq 2n$ and there exists $\alpha_1, \ldots, \alpha_t \in \R$ such that for any cut $(S, V \setminus S)$,
\[
\IVal_{M, G}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C_i}(S, V \setminus S).
\]
\end{lemma}
\begin{proof}

Note that if two strongly  $M$-connected components intersect, one of them is contained inside the other, and the smaller one has higher connectivity. Therefore, the set of all strongly $M$-connected components is a laminar family, therefore its size $t$ is at most $2n$.

Let $k_1, \ldots, k_h$ be all of the different strong $M$-connectivity values in $G$ in increasing order, and $k_0 = 0$. For $i \in [t]$, consider the component $C_i$. Suppose that it's connectivity is $k_{h_i}$. Let $C_j$ be the minimal by inclusion component containing $C_i$, and let $k_{h_j}$ be it's strong $M$-connectivity. If it exists, we set $\alpha_i = k_{h_i} - k_{h_{j}}$, otherwise $\alpha_i = k_{h_i}$.

Let $I \in \MG GM$ be an arbitrary motif instance. Notice that all of the strongly $M$-connected components containing $I$ must be nested. Let $k_{h_1}, \ldots, k_{h_j}$ be the strong $M$-connectivities of those components in increasing order, and let $k_{h_0} = 0$. Then $k_{h_j} = \kappa_I$. Therefore, by the assignment of $\alpha_i$, the following holds:
\[
    \sum_{i: I \in \MG{C_i}{M}} \frac{\alpha_i}{\kappa_I} = \sum_{i = 1}^{j} \frac{k_{h_i} - k_{h_{i - 1}}}{\kappa_I} = 1.
\]
Now, consider an arbitrary cut $(S, V \setminus S)$. We have
\begin{align*}
    \sum_{i = 1}^{t} \alpha_i \IVal_{C_i}(S, V \setminus S)&= \sum_{i = 1}^{t} \sum_{I \in \MG {C_i}{M}: I \text{ crosses } (S, V \setminus S)}  \frac{\alpha_i \cdot  w_\M(I)}{ \kappa_I} \\
    &= \sum_{I \in \MG {G}{M}: I \text{ crosses } (S, V \setminus S)}  w_\M(I) \sum_{i: I \in \MG{C_i}{M}} \frac{\alpha_i}{ \kappa_I}\\
    &=\sum_{I \in \MG {G}{M}: I \text{ crosses } (S, V \setminus S)} w_\M(I) \\
    &= \Val_{M, G}(S, V \setminus S). \qedhere
\end{align*}
\end{proof}

Now, our goal is to show the concentration result for a single strongly $M$-connected component.
There are two well-known results for hypergraph cuts that can be adapted for the case of motifs that we need to use to do that. We include the proof of one of them for completeness and show reduction of the other in a later section.

\begin{lemma}[Reformulation of Theorem 6.8 of \cite{chekuri2018minimum}]
\label{lem:weighted_cut_size}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
 If minimum of $
 \IVal_{M, G}$ of all cuts is greater than $0$, it is equal to $1$.
\end{lemma}
\begin{proof}
Let $(S, V \setminus S)$ be the cut with minimum motif size and let $k$ be the strong $M$-connectivity of $G$. Then all of the motif instances crossing the cut have connectivity exactly $k$. On the other hand, the size of cut is $k$, which gives us
\[
\IVal_{M, G}(S, V \setminus S) = 
\sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S) } \frac{w(I)}{\kappa_I} = \frac{\Val_{M, G}(S, V \setminus S)}{k} = 1. 
\]
Consider any other cut $(S, V \setminus S)$ of motif size $k'$. Then the strength of all motif instances crossing this cut is at most $k'$, which means that:
\[
\IVal_{M, G}(S, V \setminus S) = \sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S) } \frac{w(I)}{\kappa_I} \geq \frac{\Val_{M, G}(S, V \setminus S)}{k'} = 1.
\]
Therefore, the cut with the minimum motif size is the cut with the minimum value of $\IVal_{M, G}$, and the latter is equal to $1$. 
\end{proof}

\begin{lemma}[Motif Cut Counting, Reformulation of Theorem 3.2 of \cite{kogan2015sketching}]
\label{cor:cut_counting}
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph. Let $c$ be the minimum value of $\IVal_{M, G}$ across all cuts in $G$. There are at most $O(2^{
(\alpha + 1) r} n^{2(\alpha + 1)})$ cuts with value $\IVal_{M, G}$ at most $\alpha c$ for a real $\alpha \geq 1$.
\end{lemma}
The proof is given in \cref{sec:str_est}.


\begin{lemma}[Azuma's Inequality, \cite{azuma1967weighted}]
\label{lem:azuma}
Let $Z_0, Z_1, \ldots, Z_n$ be a martingale satisfying $|Z_i - Z_{i-1}| \le c_i$ for each $i \in [n]$. For any $\lambda > 0$,
\[ \p(|Z_n - Z_0| \ge \lambda) \le 2 \exp\left( \frac{-\lambda^2}{2(c_1^2 + \cdots + c_n^2)} \right). \]
\end{lemma}
We will use this lemma with a special `edge-exposure' martingale, which will be defined in \cref{lem:layer_concentration}.

The following lemmas use the values $\IVal_{M, G}$ in graph before and after sparsification by \parspar{}. To compute them, we only use the values of motif instance strength in the graph before the sparsification.

\begin{lemma}
\label{lem:layer_concentration}
Let $C$ be a strongly $M$-connected component before the application of \textsc{PartialSparsification} and $C'$ be that subgraph after the application. The following holds with probability at least $1 - n^{-c_1 }$:

Let $V_C = V(C)$. For all cuts $(S, V_C \setminus S)$ of $C$,
$$
    (1 - \epsilon') \IVal_{M, C}(S, V_C \setminus S) \leq \IVal_{M, C'}(S, V_C \setminus S) \leq (1 + \epsilon') \IVal_{M, C}(S, V_C \setminus S).
$$
\end{lemma}
\begin{proof}
By applying \cref{lem:weighted_cut_size} to $C$, we get that the minimum of values $\IVal_{M, C}$ across all cuts in $C$ is $1$.

Note that all of the critical edges in $C$ are critical in $G$, since their $M$-importance weight in $C$ is not larger than in $G$.
Since, by \cref{lem:crit_correct}, $E_+$ contains all critical edges in $G$, it also contains all of the critical edges in $C$, and, therefore, no critical edges are being sampled afterwards.
Fix a cut $(S,V_C\setminus S)$ with $\IVal_{M, C}(S,V_C\setminus S)=\alpha \geq 1$ in $C$. Let $E_2$, $t:=|E_2|$, be the set of all edges that are being sampled in \textsc{PartialSparsification} with probability $p=2^{-1/{(2r^*_{max})}} \geq 2^{-1/{(2r^*)}}$ and that are part of at least one motif cut by $(S, V_C \setminus S)$. Then $E_2$ doesn't contain any critical edges. Let $I_0$ be the subgraph of $C$ contain all vertices and edges that are a part of some motif  that is being cut by $(S, V_C \setminus S)$.

Consider the following random process: enumerate the edges in $E_2$ in the order they are being examined by \textsc{PartialSparsification}. Suppose edge $e$ with number $i$ is being sampled. If $e$ is not sampled, then we define $I_i$ to be equal to $I_{i-1}$ without $e$, otherwise $I_i$ is equal to $I_{i-1}$ with $e$ with it's weight multiplied by $1/p$. Now consider a random process $X_i$, $i \in \{0, \ldots, t\}$, where $X_i$ is equal to $\IVal_{M, I_i}(S, V_C \setminus S)$. 

It is easy to see that $X_t = \IVal_{M, C'}(S, V_C \setminus S)$ and that $X_i$ is a (doob) martingale. Let 
\[
\M^S(e) = \sum_{I\in\MG{C}{M}: e \in E(I) \land I \text{ interect} (S, V_C \setminus S) } \frac{w_\M(I)}{\kappa_I}.
\]
Then $|X_i - X_{i - 1}| \leq \M^S(e)/p^{r^*}$, where $e$ is the edge being sampled on step $i$, since the weight of all motifs can change by at most $1/p^{r^*}$ during the random process. Therefore, to apply \cref{lem:azuma}, we need to bound $\sum_{e \in E_2} \M^S(e)^2$.

Since there are no critical edges in $E_2$, for all edges $e$ that we sample, we must have 
\[\M^S(e) \leq \frac{d \epsilon'^2}{r^* (\log n + r)}.\] 
On the other hand,
\[
    \sum_{e \in E_2} \M^S(e) \leq r^* \sum_{I\in\MG{C}{M}: I \text{ interect} (S, V_C \setminus S) } \frac{w_\M(I)}{\kappa_I} = r^* \alpha,
\]
since every motif contains at most $r^*$ edges. Therefore, using this inequality:
\[  
\sum_{e \in E_2} \M^S(e)^2 \le \frac{d \epsilon'^2 }{r^* (\log n + r)} \sum_{e \in E_2} \M^S(e) \le \frac{\alpha d \epsilon'^2 }{\log n + r}.
\]
Hence, because $\IVal_{M,C}(S, V_C \setminus S) = \alpha$, by \cref{lem:azuma},
\begin{align*}
    &\p(|\IVal_{M,C}(S, V_C \setminus S) - \IVal_{M,C'}(S, V_C \setminus S)| \geq \epsilon' \IVal_{M,C}(S, V_C \setminus S)) \leq \p(|X_t - X_0| \ge \epsilon' \alpha)  \\
    &\le 2 \exp\left( \frac{-(\epsilon' \alpha )^2}{2\sum_{e \in E_2}\M^S(e) / p^{2r^*}} \right) \le 2 \exp\left( \frac{-(\epsilon' \alpha)^2}{4 \cdot \frac{\alpha d \epsilon'^2 }{\log n + r}} \right) = 2 \exp\left( \frac{-\alpha (\log n + r)}{4 d} \right).
\end{align*}

We now apply a union bound on all cuts $(S, V_C \setminus S)$ in conjunction with \cref{cor:cut_counting}. We need to bound $\sum_{\alpha \geq 1} P(\alpha)g(\alpha)$, where $P(\alpha)$ is the probability that the inequalities in the statement of the lemma doesn't hold for the cut with $\IVal_{M, C}$ equal to $\alpha$, $g(\alpha)$ is the number of those cuts, and the sum is taken across all values of $\alpha$ that are present in the graph.

Let $F(\alpha) = \sum_{\alpha \geq \alpha' \geq 1} g(\alpha')$ be the total number of cuts with $\IVal_{M, C} \leq \alpha$. By \cref{cor:cut_counting}, $F(\alpha) = A 2^{(\alpha + 1)r} n^{2(\alpha + 1)}$ for some constant $A$. We then adversarialy extend $F(\alpha)$ in a to the whole $\R_+$ such that $F(\alpha)$ is differentiable while preserving the above inequality.

We have that
\[
\sum_{\alpha \geq 1} P(\alpha)g(\alpha) \leq \int_{1}^\infty P(\alpha) \frac{dF(\alpha)}{d\alpha} d \alpha.
\]
Therefore, by applying partial integration
\begin{align*}
&\int_{1}^\infty P(\alpha) \frac{dF(\alpha)}{d\alpha} d \alpha = \Big[ P(\alpha) F(\alpha)  \Big]_{1}^{\infty} - \int_{1}^\infty F(\alpha) \frac{dP(\alpha)}{d\alpha} d \alpha\\
&\leq 2 A 2^{2r} n^4 \exp \left(-\frac{\log n + r}{4d}\right) + 
\int_{1}^\infty A n^{2(x + 1)} 2^{r(x + 1)} \frac{\log n + r}{4d} 2\exp \left(-\frac{x (\log n + r)}{4d} \right) dx \\
&\leq n^{-c_1 }
\end{align*}
by setting $d$ to be sufficiently small. Thus, the inequalities in the lemma statement hold with probability at least $1 - n^{-c_1 }$ for all cuts, as desired.
\end{proof}

We will now use the fact that for a given cut, we can take the weighted sum of the $\IVal_{M, C}$ of cuts of each of the connectivity components $C$ such that this sum is equal to the motif cut size in the whole graph. We can then apply \cref{lem:layer_concentration} to each term to obtain the cut preservation property for the whole graph.

\begin{lemma}
\label{lem:cut_component_preservation}
Let $G'$ be $G$ after the application of \textsc{PartialSparsification}. $G'$ is $(M, \e')$-motif cut sparsifier of $G$ with probability $1 - n^{-c_1 + 3}$.

\end{lemma}
\begin{proof}
By definition of motif cut sparsifier, it is enough to show that the following holds for all cuts $(S, V \setminus S)$ of $G$:
\[
    (1 - \epsilon')\textup{Val}_{M, G}(S, V \setminus S) \leq \textup{Val}_{M, G'}(S, V \setminus S) \leq (1 + \epsilon') \textup{Val}_{M, G'}(S, V \setminus S).
\]
By \cref{lem:component_sum},  we have $t \leq 2 n$ and there exist $\alpha_i \in \R$, $i \in [t]$, such that for any cut $(S, V \setminus S)$,
\[
\textup{Val}_{M, G}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C_i}(S, V \setminus S).
\]
Let $C'_i$ be $C_i$ after the application of \textsc{PartialSparsification}.
Then, similarly, the following holds:
\[
\Val_{M, G'}(S, V \setminus S) = \sum_{i = 1}^{t} \alpha_i \IVal_{M, C'_i}(S, V \setminus S).
\]
By applying \cref{lem:layer_concentration} to all $C_i$ and a union bound,  the following holds for all $i \in [t]$:
\[
    (1 - \epsilon')\IVal_{M, C'_i}(S, S \setminus V) \leq \IVal_{M, C_i}(S, S \setminus V) \leq (1 + \epsilon') \IVal_{M, C'_i}(S, S \setminus V)
\]
with probability at least $1 -  2 n^{-c_1 + 1} \geq 1 -  n^{-c_1 + 3}$.

Combining all of the equalities and inequalities, we get the claim.
\end{proof}

\subsection{Hypergraphs}
We introduce hypergraphs here since we will use some results concerning them. A hypergraph is the pair of two sets $(V, F)$, where $V$ is the set of vertices and $F$ is the set of hyperedges $f$, which are subsets of $V$. Weighted hypergraph $H=(V, F, w)$ is a hypergraph with weight function $w: F \to \R_+$.
A hypergraph $H$ is $r$-uniform if every $f \in F$ satisfies $|f| = r$.
We denote the size of the cut $(S, V \setminus S)$ in hypergraph $H$ as $\textup{Val}_H(S, V \setminus S)$.

\begin{definition}[Induced Subhypergraph]
A hypergraph $H'=(V', F', w')$ is an induced subhypergraph of a hypergraph $H=(V, F, w)$, if $V' \subseteq V$, $F' = \{ f \in F: f \subseteq V' \}$ and $w$ and $w'$ are equal on $F'$.
\end{definition}

We will abuse the cut notation for the hypergraphs: if $H'=(V', F', w)$ is an induced subhypergraph of $H=(V, F, w)$, then $\textup{Val}_{H'}(S, V \setminus S) := \textup{Val}_{H'}(S \cap V', V' \setminus S)$.

\begin{definition}[Strong Connectivity]
A weighted hypergraph $H=(V,F,w)$ is $k$-strongly connected if 
every cut $(S,V\setminus S$), $S\neq \emptyset$, $S\subsetneq V$, in $H$ has size at least $k$.
\end{definition}
 
\begin{definition}[Strongly $k$-connected Component]
\label{def:kconnectedcomp}
For a weighted hypergraph $H=(V, F, w)$ with non-negative hyperedge weights and a value $k\in \R_+$, an induced subhypergraph $C=(V_C,F_C, w)$ of $H$ is called a strongly $k$-connected component of $H$,
if 
\begin{enumerate}[label=(\alph*)]
    \item $C$ is strongly $k$-connected and,
    \item there is no induced subhypergraph $C'=(V_{C'},F_{C'}, w)$ of $G$ that is strongly $k$-connected and has $V_C \subsetneq V_{C'}$.
\end{enumerate}
\end{definition}

\begin{definition}[Hyperedge Strength]
Let $H=(V, F, w)$ be a weighted hypergraph with non-negative hyperedge weights. A hyperedge $f \in F$ has strength $\kappa_f$ if $\kappa_f$ is the
maximum value of $k$ such that there exists a strongly $k$-connected component of $H$ that contains $f$.
\end{definition}

\subsection{Strength Estimation and Motif Cut Counting}
\label{sec:str_est}
To reiterate, construction of motif cut sparsifier is not possible by only using the techniques for constructing hypergraph sparsifier. But, the problems are sufficiently close to share some similarities, which allows us to use some results for hypergraph cut sparsification in our proof.

In this section we will present omitted proofs of \cref{lem:strength_est} and \cref{cor:cut_counting} by reducing them to similar existing results for hypergraphs.

Because motif instances are essentially just subsets of vertices, it is useful to consider them as hyperedges of some hypergraph, which we will call a motif hypergraph. Note that some motif instances share the same set of vertices. In this case, the weight of the resulting hyperedge is equal to the sum of their weights.

\begin{definition}[Motif Hypergraph]
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Then the $\M$-motif hypergraph of $G$ is an undirected weighted hypergraph $H_\M=(V, F_\M, w_\M)$, where
\begin{itemize}
    \item $F_M = \{ V(I): I \in \MG GM \}$,
    \item for $f \in F_M$, $w_M(f) = \sum_{I \in \MG G M: f = V(I)} w(I)$.
\end{itemize}
\end{definition}

Note that the motif hypergraph represents the motif connectivity structure of a graph: for a cut $(S, V \setminus S)$ in $G$, its motif size is equal to it's size in $H$, and for a $I \in \MG GM$, $\kappa_I = \kappa_{V(I)}$ where $V(I)$ is a hyperedge of motif hypergraph. The introduction of hypergraph allows us to use several results from hypergraph cut sparsification, as well as giving a new perspective on the problem.

% \begin{lemma}
% \label{lem:spars_def_alt}
% Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ and $G'=(V, E', w')$ be directed weighted graphs.
% Let $H$ and $H'$ be the $M$-motif hypergraphs of $G$, $G'$.
% $G'$ is $(M, \e)$-motif cut sparsifier iff for any cut $(S, V \setminus S)$ of $H$ the following holds:
% \[
%     (1 - \epsilon) \textup{Val}_{H}(S, V \setminus S) \leq \textup{Val}_{H'}(S, V \setminus S) \leq (1 + \epsilon) \textup{Val}_{H}(S, V \setminus S).
% \]
% \end{lemma}
% \begin{proof}
% The lemma follows from the fact that the motif size of the cut $(S, V \setminus S)$ in $G$ is equal to the size of this cut in $H$, and same for the $G'$ and $H'$.
% \end{proof}

We now prove \cref{lem:strength_est} by using the following result.

\begin{lemma}[Theorem 6.1 of \cite{chekuri2018minimum}, Strength Estimation]
\label{lem:strength_est_hyper}
There exists algorithm \textsc{StrengthEstimation} which does the following:
it receives as an input a rank $r$ weighted hypergraph $H=(V, F, w)$ on $n$ vertices and outputs strength estimations $\kappa'_f$ for each hyperedge $f$ with the following properties:
\begin{enumerate}
    \item For all $f \in F$, $\kappa'_f \leq \kappa_f$,
    \item $\sum_{f \in F} \frac{w(s)}{ \kappa'_f} \leq cr(n - 1)$, for some constant $c > 0$.
\end{enumerate}
The running time of the algorithm is $O(r|F| \log^2 n \log (r |F|))$.
\end{lemma}

Note that although the algorithm presented in \cite{chekuri2018minimum} can only work with natural weights, we can easily reduce the general case to it by dividing all of the weights by the minimum one and then rounding them down to the nearest integer: tt only worsens the second property by a factor of $2$.

\begin{proof}[Proof of \cref{lem:strength_est}]
We construct motif hypergraph $H_M$ and run the algorithm from \cref{lem:strength_est_hyper} on it, then set $\kappa'_I := \kappa'_{V(I)}$ for $I \in \MG GM$. Since the construction of $H_M$ takes only $O(|\MG GM|)$ time, the total runtime is the same as in \cref{lem:strength_est_hyper}, and both properties straightforwardly follow from properties of $H_M$.
\end{proof}

Finally, we give the proof of \cref{cor:cut_counting}.

\begin{lemma}[Cut Counting in Hypergraphs, Theorem 3.2 of \cite{kogan2015sketching}]
\label{lem:cut_counting_hyper}
In an $r$-uniform weighted hypergraph $H=(V, M, w)$ with size of minimum cut $c$, there are at most $O(2^{
\alpha r} n^{2\alpha})$ cuts of size no more than $\alpha c$ for a half-integer $\alpha \geq 1$ where $\alpha$ is a half-integer if $2 \alpha$ is an integer.
\end{lemma}

\begin{proof}[Proof of \cref{cor:cut_counting}]
Consider a modification of a motif hypergraph, where each hyperedge's weight is divided by its strength. Denote it by $H'$.
It is easy to see that the size of an arbitrary cut $(S, V \setminus S)$ in $H'$ is equal to the $\IVal_{M, G}(S, V \setminus S)$. 
Indeed, 
\begin{align*}
     \Val_{H'}(S, V \setminus S) &= \sum_{f \in F: f \text{ crosses } (S, V \setminus S)} \frac{w_M(f)}{\kappa_f} \\
    &=\sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S)} \frac{w(I)}{\kappa_I} \\
    &= \IVal_{M, G}(S, V \setminus S).
\end{align*}
Therefore, it is enough to show that if $c$ is the size of the smallest cut in $H'$, the number of cuts of size $\alpha c$ is at most $O(2^{(\alpha + 1)r}n^{2(\alpha + 1)})$, which we achieve as follows: find the smallest half integer $\beta \geq \alpha$ and apply \cref{lem:cut_counting_hyper} to it and $H'$. The result then follows from the fact that $\beta < 1 + \alpha$.
\end{proof}







\subsection{Hypergraphs}
We introduce hypergraphs here since we will use some results concerning them. A hypergraph is the pair of two sets $(V, F)$, where $V$ is the set of vertices and $F$ is the set of hyperedges $f$, which are subsets of $V$. Weighted hypergraph $H=(V, F, w)$ is a hypergraph with weight function $w: F \to \R_+$.
A hypergraph $H$ is $r$-uniform if every $f \in F$ satisfies $|f| = r$.
We denote the size of the cut $(S, V \setminus S)$ in hypergraph $H$ as $\textup{Val}_H(S, V \setminus S)$.

\begin{definition}[Induced Subhypergraph]
A hypergraph $H'=(V', F', w')$ is an induced subhypergraph of a hypergraph $H=(V, F, w)$, if $V' \subseteq V$, $F' = \{ f \in F: f \subseteq V' \}$ and $w$ and $w'$ are equal on $F'$.
\end{definition}

We will abuse the cut notation for the hypergraphs: if $H'=(V', F', w)$ is an induced subhypergraph of $H=(V, F, w)$, then $\textup{Val}_{H'}(S, V \setminus S) := \textup{Val}_{H'}(S \cap V', V' \setminus S)$.

\begin{definition}[Strong Connectivity]
A weighted hypergraph $H=(V,F,w)$ is $k$-strongly connected if 
every cut $(S,V\setminus S$), $S\neq \emptyset$, $S\subsetneq V$, in $H$ has size at least $k$.
\end{definition}
 
\begin{definition}[Strongly $k$-connected Component]
\label{def:kconnectedcomp}
For a weighted hypergraph $H=(V, F, w)$ with non-negative hyperedge weights and a value $k\in \R_+$, an induced subhypergraph $C=(V_C,F_C, w)$ of $H$ is called a strongly $k$-connected component of $H$,
if 
\begin{enumerate}[label=(\alph*)]
    \item $C$ is strongly $k$-connected and,
    \item there is no induced subhypergraph $C'=(V_{C'},F_{C'}, w)$ of $G$ that is strongly $k$-connected and has $V_C \subsetneq V_{C'}$.
\end{enumerate}
\end{definition}

\begin{definition}[Hyperedge Strength]
Let $H=(V, F, w)$ be a weighted hypergraph with non-negative hyperedge weights. A hyperedge $f \in F$ has strength $\kappa_f$ if $\kappa_f$ is the
maximum value of $k$ such that there exists a strongly $k$-connected component of $H$ that contains $f$.
\end{definition}

\subsection{Strength Estimation and Motif Cut Counting}
\label{sec:str_est}
To reiterate, construction of motif cut sparsifier is not possible by only using the techniques for constructing hypergraph sparsifier. But, the problems are sufficiently close to share some similarities, which allows us to use some results for hypergraph cut sparsification in our proof.

In this section we will present omitted proofs of \cref{lem:strength_est} and \cref{cor:cut_counting} by reducing them to similar existing results for hypergraphs.

Because motif instances are essentially just subsets of vertices, it is useful to consider them as hyperedges of some hypergraph, which we will call a motif hypergraph. Note that some motif instances share the same set of vertices. In this case, the weight of the resulting hyperedge is equal to the sum of their weights.

\begin{definition}[Motif Hypergraph]
Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ be a directed weighted graph.
Then the $\M$-motif hypergraph of $G$ is an undirected weighted hypergraph $H_\M=(V, F_\M, w_\M)$, where
\begin{itemize}
    \item $F_M = \{ V(I): I \in \MG GM \}$,
    \item for $f \in F_M$, $w_M(f) = \sum_{I \in \MG G M: f = V(I)} w(I)$.
\end{itemize}
\end{definition}

Note that the motif hypergraph represents the motif connectivity structure of a graph: for a cut $(S, V \setminus S)$ in $G$, its motif size is equal to it's size in $H$, and for a $I \in \MG GM$, $\kappa_I = \kappa_{V(I)}$ where $V(I)$ is a hyperedge of motif hypergraph. The introduction of hypergraph allows us to use several results from hypergraph cut sparsification, as well as giving a new perspective on the problem.

% \begin{lemma}
% \label{lem:spars_def_alt}
% Let $\M=(V_\M,E_\M)$ be a motif and $G=(V,E, w)$ and $G'=(V, E', w')$ be directed weighted graphs.
% Let $H$ and $H'$ be the $M$-motif hypergraphs of $G$, $G'$.
% $G'$ is $(M, \e)$-motif cut sparsifier iff for any cut $(S, V \setminus S)$ of $H$ the following holds:
% \[
%     (1 - \epsilon) \textup{Val}_{H}(S, V \setminus S) \leq \textup{Val}_{H'}(S, V \setminus S) \leq (1 + \epsilon) \textup{Val}_{H}(S, V \setminus S).
% \]
% \end{lemma}
% \begin{proof}
% The lemma follows from the fact that the motif size of the cut $(S, V \setminus S)$ in $G$ is equal to the size of this cut in $H$, and same for the $G'$ and $H'$.
% \end{proof}

We now prove \cref{lem:strength_est} by using the following result.

\begin{lemma}[Theorem 6.1 of \cite{chekuri2018minimum}, Strength Estimation]
\label{lem:strength_est_hyper}
There exists algorithm \textsc{StrengthEstimation} which does the following:
it receives as an input a rank $r$ weighted hypergraph $H=(V, F, w)$ on $n$ vertices and outputs strength estimations $\kappa'_f$ for each hyperedge $f$ with the following properties:
\begin{enumerate}
    \item For all $f \in F$, $\kappa'_f \leq \kappa_f$,
    \item $\sum_{f \in F} \frac{w(s)}{ \kappa'_f} \leq cr(n - 1)$, for some constant $c > 0$.
\end{enumerate}
The running time of the algorithm is $O(r|F| \log^2 n \log (r |F|))$.
\end{lemma}



Note that although the algorithm presented in \cite{chekuri2018minimum} can only work with natural weights, we can easily reduce the general case to it by dividing all of the weights by the minimum one and then rounding them down to the nearest integer: tt only worsens the second property by a factor of $2$.

\begin{proof}[Proof of \cref{lem:strength_est}]
We construct motif hypergraph $H_M$ and run the algorithm from \cref{lem:strength_est_hyper} on it, then set $\kappa'_I := \kappa'_{V(I)}$ for $I \in \MG GM$. Since the construction of $H_M$ takes only $O(|\MG GM|)$ time, the total runtime is the same as in \cref{lem:strength_est_hyper}, and both properties straightforwardly follow from properties of $H_M$.
\end{proof}

Finally, we give the proof of \cref{cor:cut_counting}.

\begin{lemma}[Cut Counting in Hypergraphs, Theorem 3.2 of \cite{kogan2015sketching}]
\label{lem:cut_counting_hyper}
In an $r$-uniform weighted hypergraph $H=(V, M, w)$ with size of minimum cut $c$, there are at most $O(2^{
\alpha r} n^{2\alpha})$ cuts of size no more than $\alpha c$ for a half-integer $\alpha \geq 1$ where $\alpha$ is a half-integer if $2 \alpha$ is an integer.
\end{lemma}

\begin{proof}[Proof of \cref{cor:cut_counting}]
Consider a modification of a motif hypergraph, where each hyperedge's weight is divided by its strength. Denote it by $H'$.
It is easy to see that the size of an arbitrary cut $(S, V \setminus S)$ in $H'$ is equal to the $\IVal_{M, G}(S, V \setminus S)$. 
Indeed, 
\begin{align*}
     \Val_{H'}(S, V \setminus S) &= \sum_{f \in F: f \text{ crosses } (S, V \setminus S)} \frac{w_M(f)}{\kappa_f} \\
    &=\sum_{I \in \MG GM: I \text{ crosses } (S, V \setminus S)} \frac{w(I)}{\kappa_I} \\
    &= \IVal_{M, G}(S, V \setminus S).
\end{align*}
Therefore, it is enough to show that if $c$ is the size of the smallest cut in $H'$, the number of cuts of size $\alpha c$ is at most $O(2^{(\alpha + 1)r}n^{2(\alpha + 1)})$, which we achieve as follows: find the smallest half integer $\beta \geq \alpha$ and apply \cref{lem:cut_counting_hyper} to it and $H'$. The result then follows from the fact that $\beta < 1 + \alpha$.
\end{proof}
